Multi-Architecture Multi-Expert Diffusion Models

In this paper, we address the performance degradation of efficient diffusion models by introducing Multi-architecturE Multi-Expert diffusion models (MEME). We identify the need for tailored operations at different time-steps in diffusion processes and leverage this insight to create compact yet high-performing models. MEME assigns distinct architectures to different time-step intervals, balancing convolution and self-attention operations based on observed frequency characteristics. We also introduce a soft interval assignment strategy for comprehensive training. Empirically, MEME operates 3.3 times faster than baselines while improving image generation quality (FID scores) by 0.62 (FFHQ) and 0.37 (CelebA). Though we validate the effectiveness of assigning more optimal architecture per time-step, where efficient models outperform the larger models, we argue that MEME opens a new design choice for diffusion models that can be easily applied in other scenarios, such as large multi-expert models.

==> contents/bak.tex <==
% For example, the approaches of \cite{bao2022analyticdpm,liu2022pseudo,lu2022dpmsolver,salimans2022progressive,meng2022distillation,song2021denoising,song2023consistency} focus on reducing the time it takes to sample from the denoising process, whereas those of \cite{gu2022vector,ho2022cascaded,rombach2022high,vahdat2021score,tang2022improved} focus on reducing the input data size.
% post-training low-bit quantization~\cite{shang2022post} 이나, distillation~\cite{yang2022diffusion}을 통해 denoiser를 줄이려는 시도도 있었다. 그러나, 이런 방법들은 애초에 대용량의 파라미터 수를 가진 denoiser로 크게 학습시킨 모델이 있다는 전제 하에서 제안된 것이다.
% \shinhyeok{앞에 first factor 해결하려는 연구들 깐 후에 Focusing on the second factor로 연결하니까 약간 어색한 느낌이 있습니다! "Therefore, second factor에 대한 연구가 필요하다." 라는 주장을 펼치면서(first factor에서 보여줄 수 없었던 무언가가 second factor에는 있다는 내용과 함께) second factor 얘기로 넘어가면 어떨까요? }
% However, these methods are predicated on the initial presence of a substantially pre-trained diffusion model with a massive denoiser. 

% \shinhyeok{However로 연결되었다는 건 some efforts reduce the size of the denoiser에 대한 문제를 제기할 것 같은 느낌의 접속사인데 these methods are predicated on the initial presence로 넘어가는 건 문제 제기가 직접적으로 안 나와서 어색한 것 같습니다..!}

% \hist{abstract 에서는 겁나 high-low 만 외치다가 여기서는 computation cost로 시작하는게 어색한 것 같슴다. abstract 에서도 비슷한 흐름이 있어야 할 것 같아요. }
% \mh{위에서 2번 문제에 대해 주목하지 않았다고 주장했는데, 아래에서 주장하시는 문제는 그것과 크게 상관이 없어 보입니다.}
% \mh{2번 문제에 대해서, MEME가 다른 어프로치에 비해 특별히 가져가는 장점을 어필하기가 좀 어렵다는 생각이 듭니다(수많은 denoiser model 경량화 방법 중 왜 굳이 MEME이여야 하는지?). computation cost를 주요 문제로 가져가기 보다는, "Diffusion의 각 time-step에 따라 필요한 기능이 다른데, single denoiser에게 모든 것을 맡기려면 denoiser의 사이즈가 커져야 할 뿐만 아니라, multi-task learning으로 인한 성능 하락 이슈가 있다" 라는 식으로 제안하면 어떨까요? multi-expert의 필요성을 높이고, computational cost를 sub problem으로 낮추는게 목적입니다. }
% \yunsung{문단2: 이전 접근 방식과 달리, 우리의 목표는 diffusion process를 보다 능숙하게 처리하는 architecture를 찾아 높은 매개변수 denoiser 를 사용하는 diffusion models 의 한계를 극복하는 것입니다. 우선, 우리는 이전의 디퓨전 모델이 큰 파라미터를 가질 수 밖에 없던 이유가 각각의 time-step 마다 모델이 배워야할 functionality가 frequency 관점에서 매우 상이했기 때문임을 밝힌다. 우리는 실험적으로 디퓨전 모델이 time-step이 증가함에 따라 relative log amplitudes of Fourier transformed feature map의 큰폭으로 경향성있게 달라져감을 보인다. 이에 더해, 이전에는 plug-and-play guidance모델에 활용되거나, architecture capacity를 키우는데 활용되었던 multi-expert strategy가 각 구간별로 상이한 frequency관점의 functionality를 더 효율적으로 배우게 만드는 데에도 효과적일 수 있음을 보인다.}

==> contents/myeongho_1_introduction.tex <==
\section{Introduction}

Diffusion models~\cite{sohl2015deep,song2019generative,ho2020denoising} are a promising approach to generative modeling, and they are likely to play an increasingly important role in a variety of applications, including image~\cite{dhariwal2021diffusion,ramesh2022hierarchical,saharia2022photorealistic,rombach2022high,balaji2022ediffi}, audio~\cite{kong2021diffwave,popov2021grad,huang2022fastdiff,kim2022guided}, video~\cite{ho2022video,ho2022imagen,zhou2022magicvideo}, and 3D generation~\cite{poole2022dreamfusion,zeng2022lion,seo2023let}.
Despite their impressive performance, diffusion models suffer from high computation costs.
One of the contributing factors to this high computation cost is the large size of the denoiser used in traditional diffusion models.
To mitigate the massive denoiser, some efforts reduce the size of the denoiser using techniques such as post-training low-bit quantization~\cite{shang2022post} and distillation~\cite{yang2022diffusion}.
However, these methods still rely on resource-intensive training as it presupposes the existence of a pre-trained diffusion model containing a massive denoiser.

In contrast to prior approaches, our goal is to overcome the limitations of diffusion models with massive denoisers by identifying an architecture and training procedure that is more adept at handling the diffusion process.
By doing so, we can train compact diffusion models from scratch, eliminating the dependence on pretrained massive models that require significant resources.
\shinhyeok{By doing so와 can은 빼는 게 자연스럽지 않을까 싶습니다.}
\shinhyeok{We train compact diffusion models from scratch, eliminating the dependence on pre-trained massive models that require significant resources.}
First, we reveal why traditional diffusion models require massive parameters: from a frequency perspective, they must learn significantly different features in varying time-steps.
We provide empirical evidence supporting the theoretical explanation put forth by \cite{yang2022diffusion}.
They assume the denoiser network as a linear filter and demonstrate that during the denoising process, diffusion models initially form low-frequency components such as the overall image contour, and subsequently fill in high-frequency components like detailed textures.
In practice, a denoiser network has the complexity of a neural network, rather than a linear filter, and requires empirical validation of the actual training behavior.
Our investigation begins by observing the Fourier spectrum of the input $x_t$ at each time-step $t$ during the diffusion process.
We find that the spectrum loses high-frequency features as $t$ increases, a difference that becomes particularly striking at the extremes when $t$ is near initial time-step $0$ or the maximum time-step $T$.
By feeding inputs with distinctly different spectra at each $t$ into a pre-trained large denoiser model, we observe the changes in the Fourier-transformed features of each layer in the model.
\mh{제가 잘 이해를 못해서 그럴 수도 있는데, 이 부분 순서가 정리 안된 느낌입니다. (1) 결론: time-step에 따라 frequency feature가 다름 (2) 방법 (3) 결론: time-step에 따라 frequency feature가 다름.} \yunsung{요건 제가 좀 이해가 안될만하게 적은 거 같네요 고칠게여}
\mh{이 부분을 싹 묶어서 "입력을 주고 각 레이어의 fourier-transformed feature를 관측함으로써, time-step에 따라 frequency feature가 다른 것을 확인했다" 정도로 작성하면 어떨까요? } \yunsung{이렇게 묶어야 이해잘 될듯 ㅇㅇ} \shinhyeok{저도 동감이요. First, 부터 전개 순서가 좀 바뀌면 좋을 것 같습니다}
Our experimental results highlight significant and consistent variations in the relative log amplitudes of the Fourier-transformed feature maps as $t$ progresses.
This finding indicates that the costly training process of large models indeed involves learning to adapt to the different frequency characteristics at each time-step $t$.

\input{figure_tex/main_schema}

Based on these observations, we formulate the following hypothesis: \textit{By structuring the denoiser model with operations that vary according to each time-step interval, it could potentially enhance the efficiency of the diffusion model's learning process.}
To substantiate this, we introduce the novel multi-architecture strategy, wherein each architecture is assigned to its own time-step interval, composed of operations adept for their respective frequency range within the time-step intervals.
Specifically, we leverage the insights gained from \cite{d2021convit,dai2021coatnet,park2022how,si2022inception,wu2021cvt} conducted since the advent of the Vision Transformer~\cite{dosovitskiy2021an}, which reveal that convolutions are advantageous for handling high-frequency components, while multi-head self-attention (MHSA) excels in processing low-frequency components.

To enable a flexible architecture that can adapt to various frequency ranges, we propose a new denoiser architecture called iU-Net.
Our iU-Net design incorporates an iFormer~\cite{si2022inception} block that allows for adjusting the channel-wise balance ratio between the convolution operations and MHSA operations. 
We take advantage of the characteristic we discovered through our earlier observations of relative log amplitudes in Fourier-transformed feature maps, which show that diffusion models first recover low-frequency components during the denoising process and gradually add high-frequency features.
Consequently, we can configure each architecture to have a different proportion of MHSA, effectively tailoring each architecture to suit the distinct requirements at different time-step intervals of the diffusion process.

We further explore methods for effectively assigning focus on specific time-step intervals to our flexible iU-Net. Assigning distinct time-step intervals to diffusion models, referred to as the multi-expert strategy, has been applied in plug-and-play guidance models~\cite{go2022towards}, or utilized to extend model capacity by employing multiple large models~\cite{balaji2022ediffi}. However, these attempts uniformly assign a single architecture with identical operations to the experts, ignoring the fact that different operations may be more suitable at different time-steps from a frequency perspective. In contrast, our approach diversely assigns model architectures to experts so that the proportion of multi-head self-attention (MHSA) operations, which are advantageous for low-frequency components, increases as $t$ approaches $T$. We dub this novel approach Multi-architecturE Multi-Expert diffusion models (MEME). Additionally, we identify a soft interval assignment strategy for the multi-expert models that prefers a soft division over a hard segmentation. This strategy allows the experts assigned to intervals closer to $T$ to have more chance to be trained with the entire time-step.
\mh{uniform하게 time-step을 쪼개는 것에 대한 문제제기가 너무 갑작스럽게 등장한 것으로 느껴집니다. 좀 더 앞에서 한번쯤 언급을 해줘야 할 것 같습니다. 어디에...끼워야 할까...}

\yunsung{이 부분은 실험 섹션 다 채우고 다시 작성할게요}
Empirically, our MEME diffusion models successfully perform more specialized processing for each time-step interval, contributing to improved performance compared to previous baselines.
Additionally, we systematically study the design choices of the iU-Net for each expert's assigned interval to determine the most suitable configurations.
As a result, our experimental findings demonstrate that MEME outperforms the baselines on various datasets, not only in terms of generation performance but also in computational efficiency.
This is largely attributed to the efficacy of the multi-expert strategy in diffusion models, where each expert comprises only about 30\% of the parameters compared to previous models.
Consequently, our approach exhibits significantly lower computation costs compared to the previous baselines, making it a more attractive solution for real-world applications.



In summary, our contributions can be distilled into three main points:

\begin{itemize}
    \item As far as we know, we are the first to identify and address the issue that existing diffusion models rely solely on identical operations at all time-steps, despite the vastly different functionalities required at each time-step in diffusion processes.
    \item We propose MEME, a novel diffusion models framework composed of multi-architecture multi-expert denoisers which can balance operations for low-frequency and high-frequency components, performing distinct operations for each time-step interval. 
    \item MEME surpasses its counterparts not only in computational efficiency but also in terms of generation quality. Trained from scratch on the FFHQ and CelebA datasets, MEME operates 3.3 times faster than baseline models while improving FID scores by 0.62 and 0.7, respectively.
\end{itemize}

==> figure_tex/qualitative_analysis_bak.tex <==
\begin{figure*}[t]
    \centering
    \begin{tabular}{@{}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c}
        
        \raisebox{0.4\height}{\rotatebox{90}{\scriptsize Baseline}} 
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/baseline/29} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/baseline/290} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/baseline/580} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/baseline/1011} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/baseline/32} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/baseline/1700} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/baseline/2214} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/baseline/2537} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/baseline/147} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/baseline/2622} \\
        
        \raisebox{0.4\height}{\rotatebox{90}{\scriptsize MEME}} 
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/ours/29} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/ours/290} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/ours/580} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/ours/1011} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/ours/32} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/ours/1700} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/ours/2214} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/ours/2537} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/ours/147} &
        \adjincludegraphics[clip,width=0.095\textwidth,trim={0 0 0 0}]{figure_files/qualitative_analysis/ours/2622} \\
        %\footnotesize ~~~~47 & \footnotesize  69 & \footnotesize  80 & \footnotesize  118 & \footnotesize 137 & \footnotesize 164 & \footnotesize 402 & \footnotesize 439
    \end{tabular}
    \caption{Generated images by MEME and baseline.\jiny{more generated samples are illustrated in the Appendix. 라고 하고 부록에 매우 많은 생성 결과 넣어주면 좋을 것 같아요}}
    \label{fig:qualitative_analysis}
\end{figure*}





